Megaphone: Latency-conscious state migration for distributed streaming dataflows

We design and implement Megaphone, a data migration mechanism for stateful distributed dataflow engines with latency objectives. When compared to existing migration mechanisms, Megaphone has the following differentiating characteristics: (i) migrations can be subdivided to a configurable granularity to avoid latency spikes, and (ii) migrations can be prepared ahead of time to avoid runtime coordination. Megaphone is implemented as a library on an unmodified timely dataflow implementation, and provides an operator interface compatible with its existing APIs. We evaluate Megaphone on established benchmarks with varying amounts of state and observe that compared to na\"ive approaches Megaphone reduces service latencies during reconfiguration by orders of magnitude without significantly increasing steady-state overhead.

==> author_response.tex <==
\section*{Response to Reviewer Comments}

\newcommand{\rev}[1]{\emph{[Reviewer #1]}\xspace}
\newcommand{\inresponse}[1]{\textbf{Response:} #1}

We would like to thank the reviewers for their careful reading and insightful feedback. We have addressed the points raised and revised the original paper accordingly. We provide detailed answers to all revision items of the meta-review below.
\added{Changes to the document are highlighted in blue}.

\paragraph{1. Enhance experimental study (add alternative techniques \& throughput experiments)}

\stitle{Alternative techniques and comparison with related work.} We address the following specific reviewer comments:
\begin{itemize}
	\item \rev{2}\emph{W1 \& 1). No experimental comparison with related work. I think the paper can be improved by providing a better comparison with related work. The authors do cite multiple related work papers but do not discuss or experimentally evaluate any of these works in their context. For example, it is not clear how the partial pause and resume techniques discussed in section 2.1 compare with Megaphone's approach.}
	\item\rev{3}\emph{W2 \& D4). Experimental results do not include comparison with alternative techniques. I really dont see any experiments that compare with other techniques like pause/resume, stop/restaurant or even ones that use a live migration approach. Without that it is not easy to judge the actual contribution of this. Maybe the authors could add some experiments on that? Or at the very least some basic discussion on that. All-at-once seems like a baseline but given the amount of work in this area I believe more is required to establish a solid contribution.}
	\item \rev{3} \emph{D3. In the experiments I was a bit confused on that exactly is the "all-in-once" approach. Could you please add an explicit description somewhere in your experiments?}
\end{itemize}

\inresponse{Thank you for this suggestion. We realize that the original paper did not clearly present the comparison experiments and did not properly indicate that the \emph{all-at-once} migration strategy used in Section~\ref{sec:nexmark} in fact corresponds to prior work. We have made the following revisions in the paper. We have added a clarification in Section~\ref{sec:configuration} to explain that \pname's \emph{all-at-once} migration strategy corresponds to an implementation of prior techniques. We have also updated the introduction of Section~\ref{sec:evaluation} to clearly mention the comparison experiments. Finally, we have updated the results descriptions in Section~\ref{sec:nexmark} to indicate when they reflect a comparison between \pname and prior work.

As we describe in Section~\ref{sec:migration-strategies}, existing systems follow either a \emph{stop-and-restart} or a \emph{partial pause-and-resume} migration strategy (dataflow replication is not directly comparable to \pname as it requires additional resources). Further, all existing systems migrate state \emph{all-at-once}.
To perform a fair comparison, we have chosen to
implement those prior strategies in \pname itself. This allows us to use the same execution runtime across experiments and compare technique characteristics rather than specific implementations.

Our viewpoint against comparing to specific systems like Seep or Flink relies on two observations. First, these systems' JVM-based runtimes would immediately place them at a disadvantage against our Rust-based implementation. Second, published results on these systems' migration performance already exist and can be used for reference. For instance,~\cite{ds2} reports 30s downtime periods when re-configuring a Flink wordcount. 
Regarding Seep in particular, we were unable to run the publicly available code \url{https://github.com/lsds/SEEP}. After contacting the authors, we were informed that the codebase is no longer maintained and we were pointed to a re-implementation of the system, \url{https://github.com/raulcf/SEEPng}, which unfortunately does not support re-scaling at all.}

\stitle{Evaluate throughput.}
We address the following comment:
\begin{itemize}
	\item \rev{1}\emph{D6). There is not a single throughput measurement in the paper. I think it would be important to access the impact of state migration on throughput as well.}
\end{itemize}

\inresponse{Thank you for this recommendation. First, we would like to point the reviewer to our experimental setup in Section~\ref{sec:evaluation} where we describe how throughput is supplied as a parameter to our \emph{open-loop} testing harness. Nevertheless, we agree that assessing migration impact on throughput is important and we have performed a corresponding experiment. Please refer to the new Section~\ref{sec:eval:tp} and Figure~\ref{fig:keycount-migration-throughput}.}

\paragraph{2. Revise presentation}
We address the following specific comments:

\begin{itemize}
	\item \rev{1} \emph{W1). The paper is probably hard to understand if the reader is unfamiliar with timely dataflows. While the paper gives some background on timely dataflow, a Figure illustrating the frontier and the “in advance of” relation would be a useful addition.}
	\item \rev{2} \emph{W2 \& 2). The writing could be improved by introducing more examples. The paper would be an easier read if some examples are provided. For example, some examples would make sections 3.2 and 3.3 easier to read.}
	\item \rev{3} \emph{W1 \& D1). Lack of concrete examples on operators. I would like to see specific operator examples (and whole workflows) and how they are exactly reconfigured using this approach (in section 3)}
\end{itemize}

\inresponse{Thank you for the suggestion to add more examples in the paper and for pointing to specific sections which were hard to understand in the original paper. We have revised the paper to include additional examples in~\cref{sec:mechanism_guarantees,sec:configuration}. We have also highlighted and clarified the stateful word-count example in Section~\ref{sec:interface}. Finally, we have revised the description of the running example in Section~\ref{sec:example}.
}

\paragraph{3. Discuss practical considerations (when to migrate? how to integrate into other stream processing systems?)}

\stitle{When to migrate?} We address the following comment:
\begin{itemize}
	\item \rev{1}\emph{W2). Ideally, the system would take care of the migration automatically without the need for user intervention. This includes the decision of when to migrate an operator to have a fully elastic system. From my point of view, this piece is currently missing from the paper.}
\end{itemize}

\inresponse{Thank you for this insightful comment. It is indeed very important to address the issue of automatic re-configuration and some of the authors have recently worked on this topic~\cite{ds2}.
Rather than presenting a fully elastic system, our intention with \pname is to propose a generic solution to the fundamental problem of state migration: our solution can enable not only elasticity but also performance isolation, code updates, runtime optimizations and other use-cases (cf. Section~\ref{sec:introduction}). We have updated Section~\ref{sec:mechanism_overview} to mention candidate automatic controllers that could be used with \pname and explain how the configuration stream is ingested.
We have also extended the discussion in Section~\ref{sec:discussion} to highlight that \pname sets no restrictions on the controller other than the format of the control commands (cf. Section~\ref{sec:configuration})}.

\stitle{Applicability to other streaming systems.} We address the following comments:
\begin{itemize}
	\item \rev{1} \emph{D5 \& D1). Regarding the discussion of other systems: What are examples of systems that are “sufficiently expressive”? I am wondering how easy it is to implement the proposed concepts in other stream processing systems such as Spark. Storm, or Flink.}
	\item \rev{2} \emph{4). How can someone integrate the proposed mechanism into an existing streaming system? What are the changes that might be needed in the underlying system?}
	\item \rev{3} \emph{W3 \& D2). Unclear on how applicable the approach is to no timely dataflows.  I would like to see a more extended discussion (or even an example) on how this can be applied to not timely dataflows. I noticed that there a short reference to that (saying that it can be done under certain assumptions) but it is not clear to me exactly on which other types of dataflow this applies to (which satisfy your assumptions). Specifically, given that your whole Section 3 is written on the assumption that we work on timely dataflows it is very hard to envision how the reconfiguration process would apply to more general dataflows. And if this is generic then why not present it as a generic approach and then use the timely dataflows as a particular example (along with other types).}
\end{itemize}

\inresponse{Thank you for this feedback. We realize that the original paper did not properly describe when a stream processor is \emph{sufficiently expressive} to support \pname's state migration. We also agree that introducing the mechanism (Section~\ref{sec:mechanism}) on the basis of timely dataflow might leave readers with the wrong impression that \pname is specific to timely. 
We have made the following changes in the paper to address these issues. First, we have extended the introduction of Section~\ref{sec:mechanism} to better clafiy the set of system-independent features \pname relies on. In particular, we explain that basic notions of these features (support for event time, tracking computation progress, data-parallel operators, and state management) are present in all modern stream processors, such as Apache Flink, Millwheel, and Google Dataflow. Naiad and timely dataflow natively support a superset of these features and thus provide a more generic dataflow model. We thus believe that relying on the timely model as the basis to describe \pname's mechanism is useful. Second, we have extended the discussion in Section~\ref{sec:discussion} with alternative stream processor examples and we explain which of them could support \pname out-of-the-box and what additional constructs others would need to provide.
}

\paragraph{4. Address the various clarification questions raised in the reviews} We reply to each of the comments separately below.
\\
\\
\rev{1} \emph{D2: “...until they are certain that there are no other data records that could come before the record at 55.” $\to$ In general, I am wondering how the system knows that no older tuples may arrive? Tuples may always arrive out of order, and if we use event time as measure, there is no a guarantee that an older tuple arrives. Or did I misunderstand something? Please clarify.}

\vspace{2mm}
\inresponse{Thank you for this comment. In general, the streaming system is responsible to provide this guarantee via a watermark or other progress tracking mechanism. In our case, timely dataflow maintains a frontier for every operator input that specifies which timestamps can still appear on future input records (\cref{def:frontier}). We have revised the text in \cref{sec:example} to better clarify this. For further reading on fundamentals of late data handling, we would refer the reviewers to the classic streaming papers "The Design of the Borealis Stream Processing Engine" by Abadi et.~al.~and "Flexible time management in data stream systems" by Srivastava and Widom.
}
\\
\\
\rev{1} \emph{D3: The operator interfaces require a number of functions as parameters. I am wondering what the impact on efficiency is, as every function call costs performance. Are these functions inlined? Or is the network the bottleneck and the additional interpretation overhead is only marginal?}

\vspace{2mm}
\inresponse{\pname is implemented in Rust, which is very good at inlining functions passed as parameters.
We did not experience any overhead by encoding the logic as function parameters.}
\\
\\
\rev{1} \emph{D4: “The state object has to be serializable and also able to expose its elements for migration. Moreover, it has to be reconstructable from a collection of elements.” $\to$ Why does the object needs to be serializable and reconstructable? I don’t want to nit pick, but is one thing not enough for the state migration? And if so, why damanding more from a type as neccessary?}

\vspace{2mm}
\inresponse{Thank you for this question. We have rephrased the corresponding sentence in \cref{sec:implementation}.}
\\
\\
\rev{2} \emph{5) Megaphone uses two operators for state migration. How are these placed on the physical nodes? Are more resources needed?}

\vspace{2mm}
\inresponse{Thank you for this question. Timely dataflow has a copy of the whole dataflow graph on every worker/physical node.
\Cref{fig:timely_overview} shows the mapping of operators to timely workers.
\Cref{fig:mechanism_overview} visualizes how the operators for \pname are mapped to timely operators.
We added a clarifying sentence in \cref{sec:mechanism_overview}. Operators within a worker are multiplexed through cooperative scheduling: the additional operators in Megaphone do not require additional resources and introduce negligible scheduling overhead.}

\paragraph{5. Clarify relationship/improvements to prior workshop paper clearly}

We address the following comment:
\begin{itemize}
	\item \rev{2} \emph{W3 \& 3). The paper is certainly more complete than the workshop paper published by the authors but it's novelty over that one is unclear. The authors have previously published a workshop paper that describes the mechanism for state migration. The vldb submission is certainly more complete with better formalization, implementation details and more experiments. However, the novelty is a bit unclear given the previous publication.}
\end{itemize}

\inresponse{Thank you for the feedback.
According to the VLDB publication policies "A paper submitted to PVLDB must present original work not described in any prior publication that is more than 4 PVLDB-style pages in length. [...] If a PVLDB submission has overlap with a prior publication, the submission must cite the prior publication [...]". We have cited our workshop paper "Latency-conscious dataflow reconfiguration", which is 4 pages in length. To better clarify the novelty we have also expanded the text in Section~\ref{sec:introduction} to detail the new contributions in the full paper.

In particular, we extend the mechanism (\cref{sec:mechanism_guarantees}) to migrate operators that maintain a schedule of actions to perform at a later time.
We formalise the mechanisms's properties and provide a proof sketch for correctness (\cref{sec:mechanism_overview}).
We characterize the tradeoff between maximum latency and duration of a migration phase (\cref{sec:performance}), and we evaluate the latency impact under a realistic workload (\cref{sec:nexmark}).
}


==> mechanism_pseudocode_moritz.tex <==

\subsubsection{Moritz' pseudo-code!}

F operator:
\begin{lstlisting}
input: data, control
on control: stash (t, control)
check control stash:
  if control frontier !<= t in (t, control):
    - compile control
    - add to pending
check pending control:
  if data frontier !<= t in (t, pending control)
  and probe !<= t
    - migrate bins to new owner
on data: if control frontier !<= t of (t, data):
    - for each record: lookup receiver, forward tuple
 else:
    - stash (t, data)
check pending data: if frontiers !<= (t, data):
    - for each record: lookup receiver, forward tuple
\end{lstlisting}

S operator:
\begin{lstlisting}
input: data, state
in state: apply state updates
in data: stash data
check data stash: if frontiers !<= t in (t, data):
    - consume(t, data, bin)
check binned data: if frontiers !<= t (t, binned data):
    - fold(t, data, bin)
\end{lstlisting}


==> related.tex <==
\section{Related Work}
Check the following papers~\cite{Qian13,Wu15,Barker12,Das11,Elmore11,Ananthanarayanan12}.

